Round- and Message-Optimal Distributed Graph Algorithms

Distributed graph algorithms that separately optimize for either the number of rounds used or the total number of messages sent have been studied extensively. However, algorithms simultaneously efficient with respect to both measures have been elusive. For example, only very recently was it shown that for Minimum Spanning Tree (MST), an optimal message and round complexity is achievable (up to polylog terms) by a single algorithm in the CONGEST model of communication. In this paper we provide algorithms that are simultaneously round- and message-optimal for a number of well-studied distributed optimization problems. Our main result is such a distributed algorithm for the fundamental primitive of computing simple functions over each part of a graph partition. From this algorithm we derive round- and message-optimal algorithms for multiple problems, including MST, Approximate Min-Cut and Approximate Single Source Shortest Paths, among others. On general graphs all of our algorithms achieve worst-case optimal $\tilde{O}(D+\sqrt n)$ round complexity and $\tilde{O}(m)$ message complexity. Furthermore, our algorithms require an optimal $\tilde{O}(D)$ rounds and $\tilde{O}(n)$ messages on planar, genus-bounded, treewidth-bounded and pathwidth-bounded graphs.

==> deterministic.tex <==
\section{Deterministic Completion of Framework}\label{sec:deterministic}
We now present how our remaining black boxes -- star joinings and shortcuts -- can be computed in a deterministic fashion. 

\subsection{Deterministic Algorithm for Star Joinings}
In this section, we show how a star joining of node clusters, sub-part clusters and parts can be efficiently computed given that we've already shown how computation can be efficiently and deterministically computed within each of these.

We use as a symmetry-breaking primitive, the algorithm of \citet{cole1986deterministic}. Roughly the algorithm works as follows. Every node begins with its node ID as its color, meaning there are initially $n$ colors. Next, every node updates its color based on its neighbors colors in such a way that the resulting number of possible colors is logarithmically smaller. This is then repeated $\log^* n$ times. For more, see \citet{cole1986deterministic}.

\begin{lem}\label{lem:cole-vishkin}[\citet{cole1986deterministic}]
	An oriented $n$-vertex graph with maximum out-degree of one can be $3$-colored in $\log^* n + O(1)$ rounds and $O(m \log^*n)$ messages.
\end{lem}


%In this section, we discuss how to merge parts $P_i$ into new parts $P'_j$ such that the obtained parts together with their constituent parts' shortcuts induce low-diameter subgraphs. That is, if a new part $P'_j$ is the union of some set of parts $\{P_i \mid i\in I\}$ and $S'_j$ is the union of these parts' shortcuts, i.e., $S'_j=\bigcup_{i\in I} S_i$, then the diameter of $G[P'_j \cup S'_j]$ should not increase too much compared to the maximum diameter of any $G[P_i \cup S_i]$ with $i\in I$. 

%Ellis: this discussion now in preceding section
%\dwnote{paragraph should move elsewhere.} \textbf{For randomized algorithms} this is easily obtained by having each part flip an unbiased coin independently and only merging parts $P_i$ and $P_k$ with $P_i$ attempting to merge with $P_k$ if $i$'s coin came out heads and $k$'s coin came out tails. In this case every new component $P'_j$ together with its shortcut edges $S'_j$ clearly has diameter at most $D(G[P'_j \cup S'_j])\leq 3 \max_{i\in I} D(G[P_i \cup S_i]) + 2$. %This is trivial if $P'_j$ is made of precisely one part $P_i$ (i.e., $|I|=1$). If, however, $P'_j=\bigcup_{i\in I} P_i$ with $|I|>1$, then $P'_j$ contains precisely one part which tossed a tails, denoted by $P^T_i$. But then, for any two nodes $u,v$ in $P'_j$, if $u\in P_{i_1}$ and $v\in P_{i_2}$, then there exists a path from $u$ to a node in $P_{i_1}$ incident to 
%Moreover, the number of components decreases by a constant in expectation, implying that the algorithm terminates within $O(\log n)$ rounds (w.h.p).

We now state how star joinings can be efficiently and deterministically computed.
\begin{lem}
\label{lem:starJoinDet}
Let $V_1, \ldots, V_N$ be a partition of $U \subseteq V$ with each $V_i$ having a connecting edge exiting $V_i$ and a leader or representative node $l_i$.
If we can solve the part aggregation problem in each $V_i$ deterministically in $O(R)$ rounds and $O(M)$ messages, then there exists a deterministic algorithm that computes a star joining in $O(R\log^*n)$ rounds with $O(M\log^*n )$ messages.
\end{lem}

\begin{proof}
Consider the super-graph consisting of each $V_i$ as a single super-node and the chosen edges. Direct the chosen exiting edge of a $V_i$ towards the $V_j$ to which it connects. We compute our star joining in two stages.
%: in the first stage we compute our star joining for $V_i$s that form trees and in the second stage we compute our star joining for $V_i$s on the remaining cycles and paths. 
The first stage works as follows. All $V_i$s with more than one incoming edge are marked. 
A marked $V_i$ is designated a receiver and an unmarked $V_i$ whose out edge is towards a marked 
part is designated a joiner. This stage yields $V_i$s that are stars centered on marked parts. 
Moreover, the super-nodes of this stage form trees of internal degree at least 2. Therefore, the number of internal (marked) super-nodes (and therefore the number of stars) is at most one half of the super-nodes of the tree.\dwnote{cite exercise from textbook on graph theory.}
All super-nodes that are joiners or receivers in this stage are now removed from the super-graph, following which we run stage two. 
As no super-node has in-degree two, the super-graph considered in stage two consists of directed cycles and paths.

Stage two works as follows. First, we simulate the Cole-Vishkin algorithm on our super-graph as follows.
Each $V_i$ begins with the color of $l_i$'s ID. 
Next, the node in $V_i$ incident to the edge chosen by $V_i$ routes the color it received to $l_i$. Then, $l_i$ performs the Cole-Vishkin computation and then broadcasts $V_i$'s new color to all nodes in $V_i$. This is repeated $\log^* n + O(1)$ times, resulting in a 3-coloring of our super-graph. Next, for color $k=1,2,3$: every $V_i$ colored $k$ is removed from the super-graph, together with its neighbors. Every such $k$-colored $V_i$ is designated a joiner and its neighbor along its chosen edge is designated a receiver. As the super-graph consists of paths and cycles at this point, each time we remove a $V_i$ from the super-graph we remove at most three super-nodes from the graph and $V_i$ gets to merge with its neighbor. It follows that at least $\frac{1}{3}$ of these super-nodes are merged, and so the number of stars obtained is at most $2/3$ of the original number of super-nodes.

Combining the first and second stage, we find that the super-nodes are combined into stars, where
the number of obtained less than 2/3 of the nodes. Therefore the above algorithm computes a star joining.
We now bound our algorithm's round and message complexity. Each of the $O(\log^*n)$ phases of the algorithm require the transmission of a message to and/or from $l_i$ from/to every node in $V_i$, all 
implementable using the part aggregation problem as a subroutine. The claimed round and message complexities of $O(R\log^*n)$ and $O(M\log^*n)$ follow.
%: in the first stage each node has value equal to the number of incoming chosen edges it is incident on, and the function computed is the sum (allowing to verify the ). In the second stage, when simulating the Cole-Vishkin algorithm, we first have the node neighboring the out edge have value 
%As such, our algorithm can be implemented in $O(R\log^*n)$ rounds and $O(M\log^*n)$ messages, by appealing to our 
%
%It remains to argue round and message complexities of $O(R \log^* n)$ and $O(M \log ^* n)$ respectively. First, notice that the first stage takes $O(R)$ rounds and $O(M)$ messages as all that each $V_i$ needs to do is compute the number of inbound edges incident to it, alert its neighbors as to whether it is marked or unmarked and designate itself a joiner, receiver or neither as appropriate. Next, notice that the second stage requires $O(R \log^* n)$ rounds and $O(M \log^* n)$ messages. In particular, computing the 3-coloring requires $\log^*n$ rounds of routing two messages to each $l_i$, requiring $O(R \log^*n)$ rounds and $O(M \log^*n)$ messages and designating joiners, receivers and marking for each color requires $O(R)$ rounds and $O(M)$ messages.
%
%
%Lastly, we argue correctness. In particular we argue that this algorithm computes a star joining of size $sN$ for constant $0 < s < 1$. First, notice that the super-nodes removed in the first round along with their chosen edges form trees whose leaves are unmarked and whose internal nodes are marked. Thus, every leaf will successfully merge with its parent. Moreover, every internal node of each of these trees has degree at least two and so at least half of the nodes in the tree are leaves meaning at least half of the nodes in each tree are merged. 
%
%Next, we argue that the super-graph in stage two consists of only cycles and paths. Suppose for the sake of contradiction that in stage two there exists some cycle  (resp. path) of super-nodes with a super-node not in the cycle connected to a super-node in the cycle. Then this super-node would have been marked in the first stage and removed and so no such structure can exist in the second stage.
%
%Lastly, we argue that a constant fraction of each cycle and path in the second stage is merged together. Each time we remove a $V_i$ from the super-graph we remove two or three super-nodes from the graph and $V_i$ gets to merge with its neighbor. It follows that at least $\frac{1}{3}$ of these super-nodes are merged.
% By assumption this stage can be completed in $O(R)$ rounds with $O(M)$ messages. If all parts were either unmarked and connected by their chosen edge to a marked node or marked then we would be done, as we would decrease the number of $V_i$s by a constant factor \enote{This should be argued more carefully}. However, we still have to deal with directed cycles and paths. 
% 
% In addition, the number of unmarked nodes merged along their out edge in this stage is strictly greater than the number of marked nodes not merged along their edges, as these nodes form directed trees with each internal node having degree at least two.
%
%We now remove all unmarked nodes that connect to a marked node or marked nodes
%
%To deal with cycles and paths, we rely on the algorithm of \citet{cole1986deterministic} given above. In particular, we first remove all $V_i$s from 
%
%The way we use this primitive is as follows: during every round of part-growing, every part chooses some ``out'' edge along which it wishes to merge. Shrinking each part into a single node, the obtained graph has max out-degree of one. Of course, this is a little simplistic, as the nodes in this shrunken graph correspond to parts. However, the intermediate colors assigned to each node by the Cole-Vishkin algorithm only rely on the previous color, together with the ``parent'' node's previous color. Therefore, each part can delegate all the local computation to its node neighboring the ``parent'' part (the node in this part is the source of the outgoing edge to the parent part), following which this color is broadcast to all nodes in the part using the shortcuts. This reduction blows up the number of rounds of the Cole-Vishkin algorithm by the time to transmit within a part using the shortcuts \dwnote{$O(d+c)$ rounds? If so, $O((d+c)\log^*n)$ rounds in total} while requiring messages of a total of $O(n \log n)$ bits to be transmitted throughout this implementation of the Cole-Vishkin algorithm.\footnote{The Cole-Vishkin algorithm requires each node to compute a color using $\log n$ bits, then $O(\log\log n)$ bits, then $O(\log \log \log n)$ bits, and so on, and therefore each vertex only ever needs to receive $O(\log n)$ bits during these rounds.}\dwnote{what about messages sent up the shortcuts?} 
%
%Given the above 3-coloring algorithm, we compute our second stage as follows.  In each super-round a $V_i$ can compute any commutative associative function using $O(R)$ rounds and $O(M)$ messages. First, our super-graph runs the Cole-Vishkin algorithm which takes $O(R\log^* rounds)$ and $O(M \log^*)$ messages.
%
%our way to guarantee that a new part has a moderate shortcut-diameter compared to its constituent parts (while decreasing the number of parts by a constant fraction) is simple as follows. For color $i=1,2,3$, we let unmarked parts numbered(colored) $i$ merge along their chosen out-edge, and mark their neighbors. Note that the unmarked parts in this stage form a maximal independent set (MIS).
%The new parts are the union of at most three parts of the previous partition, and as such have low shortcut-diameter. On the other hand, every three parts along a directed path or cycle contain at least one unmarked part, as the set of unmarked parts constitutes an MIS.
%The new parts $P'_j$ therefore have dilation at most $3\max_{i\in I} D(G[P_i \cup S_i]) + 2$. Crucially, this symmetry-breaking guarantees that at least a third of the parts are merged into a larger part, implying that after a logarithmic number of these ``Bor\r{u}vka steps'' we obtain a single part. %\dwnote{Yes, I know we're solving a more general problem than MST...}
%\dwnote{Be consistent with terminology. Parts/sub-parts/clusters/etc'...}
%=======
%Consider the super-graph consisting of each $V_i$ as a single super-node and the chosen edges. Direct the chosen exiting edge of a $V_i$ towards the $V_j$ to which it connects. We compute our star joining in two stages: in the first stage we compute our star joining for $V_i$s that form trees and in the second stage we compute our star joining for $V_i$s on the remaining cycles and paths. 
%
%The first stage works as follows. First, all $V_i$s with more than one incoming edge are marked. A marked $V_i$ is designated a receiver and an unmarked $V_i$ whose out edge is towards a marked part is designated a joiner. This stage yields $V_i$s that are stars centered on marked parts. All super-nodes that are joiners or receivers are now removed from the super-graph and we run stage two. 
%
%Stage two works as follows. First we run the Cole-Vishkin algorithm to compute a 3-coloring of the super-graph. In particular, we simulate the Cole-Vishkin algorithm on our super-graph as follows: each $V_i$ begins with the color of $l_i$s ID. As we later argue the super-graph at this point only consists of cycles and paths. As such, each $V_i$ has at most 2 super-node neighbors, one who $V_i$ is connected to by $V_i$'s chosen edge, $V_j$, and one who connects to $V_i$ via its chosen edge, $V_k$. Next, nodes incident to connecting edges relay their colors to each other along their connecting edges. For each $V_i$, there are at most two nodes that receive a color from a neighbor and so these route the received color to $l_i$ (say the one incident to the outbound edge routes first). Next $l_i$ performs the Cole-Vishkin computation based on its neighbors colors and then broadcasts this to all nodes in $V_i$. This is repeated $\log^* n$ times, resulting in a 3-coloring of our super-graph.
%
%Next, for color $i=1,2,3$: every $V_i$ colored $i$ and its neighbors is removed from the super-graph. Every such $V_i$ is designated a joiner and its neighbor along its chosen edge is designated a receiver.
%
%It remains to argue round and message complexities of $O(R \log^* n)$ and $O(M \log ^* n + m \log^*m)$ respectively. First, notice that the first stage takes $O(R)$ rounds and $O(M)$ messages as all that each $V_i$ needs to do is compute the number of inbound edges incident to it, alert its neighbors as to whether it is marked or unmarked and designate itself a joiner, receiver or neither as appropriate all of which is achievable by computing various associative and commutative $f$s. Next, notice that the second stage requires $O(R \log^* n)$ rounds and $O(M \log^* n + m \log^*n)$ messages. In particular, computing the 3-coloring algorithm requires $\log^*n$ iterations each using $O(R)$ rounds at most $m$ messages to relay colors to neighbors and $O(M)$ messages to route to and broadcast from $l_i$s. Lastly, designating joiners, receivers and marking for each color requires $O(R)$ rounds and $O(M)$ messages.
%
%Lastly, we argue correctness. In particular we argue that this algorithm computes a star joining of size $sN$ for constant $0 < s < 1$. First, notice that the super-nodes removed in the first round along with their chosen edges form trees whose leaves are unmarked and whose internal nodes are marked. Thus, every leaf will successfully merge with its parent. Moreover, every internal node of each of these trees has degree at least two and so at least half of the nodes in the tree are leaves meaning at least half of the nodes in each tree are merged. 
%
%Next, we argue that the super-graph in stage two consists of only cycles and paths. Suppose for the sake of contradiction that in stage two there exists some cycle  (resp. path) of super-nodes with a super-node not in the cycle connected to a super-node in the cycle. Then this super-node would have been marked in the first stage and removed and so no such structure can exist in the second stage.
%
%Lastly, we argue that a constant fraction of each cycle and path in the second stage is merged together. Each time we remove a $V_i$ from the super-graph we remove two or three super-nodes from the graph and $V_i$ gets to merge with its neighbor. It follows that at least $\frac{2}{3}$ of these super-nodes are merged.
\end{proof}

As a corollary of \Cref{lem:starJoinDet}, we conclude the following.
\begin{cor}
\label{cor:starJoinDet}
Star joinings can be computed deterministically  for
\begin{enumerate}
\item Node clusters in $O(D\log^*n)$ rounds with $O(n\log^*n)$ messages by \Cref{lem:fOfClusterNodes}.
\item Sub-part clusters in $O(b(D+c)\log^*n)$ rounds and $O(m\log^*n)$ messages given a T-restricted shortcut $\mathcal{H}$ with congestion $c$ and block parameter $b$ and a sub-part division by \Cref{lem:SPClusF}
\item Parts in $O(b(D+c)\log^*n)$ rounds and $O(m\log^*n)$ messages given a T-restricted shortcut, a sub-part division and a sub-part division leader in $O(b(D+c))$ rounds and $O(n)$ messages by \Cref{thm:computePartf}.
\end{enumerate}
\end{cor}


%The following lemma summarizes the discussion of this section.
%
%\begin{lem}
%	Given $(c,d)$-shortcuts, %``an iteration of Bor\r{u}vka's algorithm'' 
%	parts can be merged within $O((c+d)\log^*n)$ CONGEST rounds, with message complexity $O(n \log n)$. \dwnote{in $O(n)$ messages? Analyze more carefully.}
%\end{lem}

%SUBSECTION: Deterministic Shortcut Construction
\subsection{Deterministic Shortcut Construction}
Having shown how star joinings can be computed in a deterministic fashion, we now turn to our deterministic shortcut construction. We rely on heavy path decompositions~\cite{sleator1983data}. 

\begin{Def}[Heavy Path Decomposition \cite{sleator1983data}]
	Given a directed tree $T$, an edge $(u,v)$ of $T$ is  \emph{heavy} if the number of $v$'s descendants is more than half the number of $u$'s descendants; otherwise, the edge is \emph{light}. A \emph{heavy path decomposition} of $T$ consists of all the heavy edges in $T$.
\end{Def}

It is immediate from the definition that each leaf-to-root path on an  $n$-node tree $T$ intersects at most $\lfloor \log_2 n\rfloor$ different paths of $T$'s heavy path decomposition.
Given a rooted tree $T$ of depth $D$, a heavy path decomposition of $T$ can be easily computed in $O(D)$ rounds using $O(n)$ messages.

To construct our $T$-restricted shortcuts, we will compute a heavy path decomposition of $T$ and then compute efficient shortcuts on the obtained paths in bottom-up order. The problem of computing shortcuts on paths, generally stated, is as follows.
\begin{Def}[The path shortcuts problem]
The input is a directed path $\mathcal{P}$ of length $D$, with each node $v$ of the path $\mathcal{P}$ ``belonging'' to a set $S(v)$ of parts, along with parameters $c$ and $b$. We wish to compute an $O(c \log D)$-congestion shortcut of $\mathcal{P}$ with block parameter $O(b)$. 
\end{Def}
For simplicity, assume vertices of $\mathcal{P}$ are numbered by their height, $v=1,2,\dots$ (i.e., the source of the path is number $1$, its parent is numbered $2$, etc'). Our algorithm will run for $\log_2D$ rounds, where at the beginning of each round $r$ we have $S_r(v)$ be the set of part IDs using $v$ via shortcut edges. The algorithm iteratively extends paths used for shortcuts, doubling them in length (unless this creates too much congestion). The algorithm is given in \Cref{alg:path-shortcut}.

\begin{figure}[h]
\begin{minipage}{.6\linewidth}
%\begin{algorithm}
%	\subcaption{Shortcut Construction on Paths}
	%	\label{alg:path-shortcut}
	\begin{algorithmic}[1]
		\medskip
		\FORALL{nodes $v$}
		\STATE $S_0(v) \leftarrow S(v)$.
		\FORALL{$r=0,1,\dots,\log_2D-1$}
			\FORALL{nodes $v\equiv 2^r \mod 2^{r+1}$, \textbf{in parallel,}}
				\IF{$|S_{r}(v)|\geq 2c$}
					\STATE break edge $(v,v+1)$.
				\ELSE
					\STATE transmit $S_{r}(v)$ towards   node $u=v+2^r$
					\\\textbackslash* stop if broken edge encountered*\textbackslash
					\IF{$S_r(v)$ reaches $u=v+2^r$}
						\STATE $S_{r+1}(u) \leftarrow S_r(u) \cup S_r(v)$.
					\ENDIF 
				\ENDIF
			\ENDFOR 
		\ENDFOR
		\ENDFOR
		\RETURN set of non-broken edges as shortcuts.
	\end{algorithmic}
%\end{algorithm}
\end{minipage}
\begin{subfigure}{.4\textwidth}
	\centering
	\includegraphics[scale=0.56]{figs/path-shortcut-algorithm-run.pdf}
	\subcaption{Illustration of a directed path and its potentially shortcut-edge-connected subpaths after rounds $0,1$ and $2$, respectively (indicated by dashed ovals).}
\end{subfigure}
\captionof{algorithm}{The deterministic shortcut construction algorithm for paths.}
\label{alg:path-shortcut}
\end{figure}

%\dwnote{Remove algorithm environment. Looks too wordy.}

The properties of this algorithm are given in the following lemma.

\begin{lem}\label{lem:path-shortcut}
	Given the existence of a $T$-restricted shortcut with congestion $c$ and a path $\mathcal{P}$ going up $T$,
	% with block number $b$ be such that there exists a low-congestion shortcut $\mathcal{H}$ of $G$ with congestion $c$ and block number $b$. Then 
	Algorithm \ref{alg:path-shortcut} computes a shortcut on $\mathcal{P}$ with congestion $O(c\log D)$ in $O(c\log D + D)$ rounds.% with $|\mathcal{P}| c \log D$ messages. % such that for at least $N/2$ parts, the number of blocks is at most $3b$.
\end{lem}
\begin{proof}
	To bound the running time, observe that round $r$ of the algorithm can be implemented in $c+2^r$ rounds.  Summing over all rounds 
	$r=0,1,\dots,\log_2 D-1$, the bound follows. 
	To bound the congestion of the output shortcuts, we prove by induction that before the $r$-th round the congestion on any edge is at most $2cr$. This clearly holds before round $r=0$. Now, before round $r$, all edges are used by at most $2cr$ parts. After round $r$ all edges $(v,v+1)$ for a node $v$ with $v\mod 2^{r+1} \in [0,2^r-1]$ have their congestion unchanged, while all edges $(v,v+1)$ for a node $v$ with $v\mod 2^{r+1} \in [2^r,2^{r+1}-1]$ have their congestion increase by at most $2c$, implying the claimed bound. %Finally, the number of messages transmitted along any of the $|\mathcal{P}|$ edges is $O(c \log D)$, implying the bound on the message complexity.
\end{proof}

The shortcuts obtained by Algorithm \ref{alg:path-shortcut} can be shown to also satisfy the property that most parts have low block number in the obtained shortcuts. Rather than proving this property for this subroutine, we turn to describing the overall shortcut construction algorithm and analyze the resulting block number there.

In order to use Algorithm \ref{alg:path-shortcut} to compute an efficient $T$-restricted shortcut, we first compute a heavy path decomposition of $T$. For every node $v$, we initialize $S(v)$ to be the singleton containing $v$'s part ID, \emph{provided $v$ is a sub-part representative}. We now run Algorithm \ref{alg:path-shortcut} in parallel for each path with no incoming light edge. Next, for each such path's sink node $v$, let $S^{final}(v)=S_{\log_2 D - 1}(v)$ be the set of part IDs which can use the edge up to $v$. If $|S^{final}(v)|\geq 2c$, break $v$'s parent edge. Else, transmit $S ^{final}(v)$ up $v$'s tree edge to $v$'s parent $u$, and update $S(u)$ accordingly, by letting $S(u)$ be the union of $S(u)$ and $S^{final}(v)$ for all light children of $v$ for which $S^{final}(v)$ was computed. Repeat the above for $\lfloor\log_2 n\rfloor$ phases, each time removing the previous phase's source paths. Finally, output the non-broken edges as a shortcut. The properties of this algorithm are given in the following lemma.

\begin{lem}\label{lem:overall-shortcut}
	Let $\mathcal{H}$ be some $T$-restricted shortcut with congestion $c$ and block number $b$. Then, given a sub-part division, the previous algorithm can be implemented in $O(c\log D \log n + D\log n)$ rounds and $O(n\log n)$ messages, outputting a shortcut $\mathcal{H}'$ with congestion $O(c\log n)$ where at least half of the parts have block number at most $O(b)$ in $\mathcal{H}'$.
\end{lem}
\begin{proof}
	As mentioned above, a heavy path decomposition of $T$ can be computed in $O(D)$ rounds using $O(n)$ messages.
	Next, note that a path $\mathcal{P}_i$ can find out whether it has a light edge in $O(D)$ rounds with $|\mathcal{P}_i|$ messages. Therefore finding the relevant parts during each phase requires a total of $O(D\log n)$ rounds and $\sum_i |\mathcal{P}_i| \cdot \log n = O(n \log n)$ messages. Next, running Algorithm \ref{alg:path-shortcut} $O(\log n)$ times requires $O(c\log D\log n + D\log n)$ rounds. To bound the message complexity of the invocations of Algorithm \ref{alg:path-shortcut} together with upcasts along light edges, we note that part IDs are only forwarded up, at most $D$ hops, and they are only forwarded from the $O(n/D)$ sub-part representatives. Consequently, the overall message complexity of the algorithm is $O(n\log n)$.	
	Finally, removing the parts dealt with at any phase can be done implicitly, by notifying each adjacent path in the following phase that this path was ``removed'', all within the time and message bounds of verifying if a path has no incoming light edges.
	
%	The running time and congestion due to running Algorithm \ref{alg:path-shortcut} are immediate from Lemma \ref{lem:path-shortcut}. 
	
	We now analyze the block number of (most of) the parts.
	Let $N$ be the number of parts and let $U$ be the set of heavy edges used in the optimal shortcut $\mathcal{H}$ but broken and therefore unusuable as part of the output shortcut. Each such edge received at least $2c-c=c$ more requests by parts to use it than in the optimal shortcut. But each part can contribute at most $b$ such additional requests to a broken edge, as each block can only send one additional request towards the tree's root. Consequently, we have $|U|\leq N\frac{b}{2c}$. Next, we say a part is \emph{bad} if greater than $2b+b\log_2 n$ of its edges of the optimal shortcut are broken, and \emph{good} otherwise. Note that for a good part the number of blocks in the output shortcut is at most $2b+b\log_2 n = O(b\log n)$. On the other hand, every broken heavy edge used in the optimal shortcuts is used at most $c$ times in $\mathcal{H}$.
	We conclude that the number of bad parts is at most $|U|\frac{c}{2b}$. Combining both upper and lower bounds on $|U|$, the number of bad parts is at most $N/2$, implying the claimed bound.
\end{proof}

Combining \Cref{cor:starJoinDet}  and \Cref{lem:stardivSPClust}, it is possible to deterministically compute which parts have block number less than $kb$ in $O(b(D+c)\log n \log^* n)$ rounds and $O(m \log^2 n \log^*n)$ messages for appropriate constant $k$. Thus, we can iterate the algorithm of \Cref{lem:overall-shortcut} logarithmically many times -- removing parts with block number less than $kb$ in each iteration -- to get the following result.

\begin{lem}
\label{lem:ScutDet}
	Given a tree $T$ of depth $D$ and parts, which admit a shortcut of congestion $c$ and block number $b$ and a sub-part division, one can compute deterministically in $O(b(c \log^3 n + D \log^2 n \log^* n))$ rounds and using $O(m \log^3 n \log^*n)$ messages, a $T$-shortcut with congestion $O(c\log n)$ and block parameter $O(b)$.
\end{lem}
%\begin{proof}
%	Repeat the previous algorithm $\log N \leq \log n$ times, each time only considering the parts with current block number greater than $3b$. The only delicate point to note is that figuring out which parts are broken may require us to broadcast using the obtained shortcuts, 
%	%The running time and congestion are immediate, while the number of parts with block number greater than $3b$ decreases by a factor of two for each repeated run of Algorithm \ref{alg:path-shortcut}. 
%\end{proof}

Combining \Cref{thm:computePartf} or \Cref{thm:MST} with the now unpacked deterministic black boxes yields the deterministic algorithm of \Cref{thm:partComputation} or \Cref{thm:mst} respectively.

%Combining \Cref{cor:starJoinDet}, \Cref{lem:ScutDet}, \Cref{lem:comDiv}, \Cref{lem:stardivSPClust}, \Cref{thm:MST} and \Cref{thm:computePartf} yields the deterministic algorithms of \Cref{thm:partComputation} and \Cref{thm:mst}.%Commenting this out because not informative




==> randomized.tex <==
\section{Randomized Completion of Framework}
\label{sec:Randomized}
In this section we unpack our remaining black boxes by describing how star joinings and shortcuts can be computed in a randomized fashion.

%SUBSECTION: Randomized Algorithm for Star Joinings
\subsection{Randomized Algorithm for Star Joinings}
\label{subsec:randStarJoing}
Given the symmetry-breaking that randomization enables, computing a star joining of node clusters, sub-part clusters or parts is easily accomplished by flipping coins and sharing randomness.

\begin{lem}
\label{lem:randStarsJoin}
Let $V_1, \ldots, V_N$ be a partition of $U \subseteq V$ with each $V_i$ having a connecting edge exiting $V_i$ and a leader or representative node $l_i$. If we can solve the partition computation problem over $V_1, \ldots, V_N$ in $O(R)$ rounds and $O(M)$ messages, then there exists a randomized algorithm that computes a star joining in $O(R)$ rounds with $O(M)$ messages.
\end{lem}
\begin{proof}
Each $l_i$ simply flips a coin and distributes this value to $V_i$. Any $V_i$ whose leader flips a heads is designated a receiver and all other $V_i$s are designated senders. In expectation, $\frac{1}{4}$ of all $V_i$ will be able to be merged.
\end{proof}

We can then conclude that a star joining of node clusters, sub-part clusters or parts is efficiently computable by combining \Cref{lem:randStarsJoin} and our earlier results that describe how each of these can perform efficient computation.
\begin{cor}
\label{cor:starJoinRand}
Star joinings can be randomly computed for

\begin{enumerate}
\item Node clusters in $O(D)$ rounds with $O(n)$ messages by \Cref{lem:fOfClusterNodes}.
\item Sub-part clusters in $O(bD+c\log n))$ rounds and $O(m)$ messages given a T-restricted shortcut with congestion $c$ and block parameter $b$ and a sub-part division by \Cref{lem:SPClusF}
\item Parts in $O(bD+c \log n))$ rounds and $O(m)$ messages given a T-restricted shortcut, a sub-part division and a sub-part division leader by \Cref{thm:computePartf}.
\end{enumerate}
\end{cor}

%SUBSECTION: Randomized Shortcut Construction
\subsection{Randomized Shortcut Construction}
\label{subsec:randSCut}

We now describe how shortcuts can be computed in few rounds with low message complexity with randomization.

%Theorem: randomized shortcut computation
\begin{thm}
\label{thm:randSCut}
Given a sub-part division, a spanning tree $T$ and the existence of a T-restricted shortcut with congestion $c$ and block parameter $b$, there exists a randomized algorithm that computes a $T$-restricted shortcut with congestion at most $8c$ and block parameter at most $3b$ in $O(bD\log^3 n + c \log^3 n)$ rounds with $O(m \log^2 n)$ messages.
\end{thm}
\begin{proof}
\citet{GoranShortcuts} provide a randomized algorithm where given $T$, a $T$-restricted shortcut with congestion at most $8c$ can be computed such that at least half of the parts have block parameter at most $3b$ in $O(D\log n + c)$ rounds. In the algorithm, every node sends a message up $T$ once leading to super-linear message complexity. See \citet{GoranShortcuts} for more details. By amending this so only the $O\left(\frac{n}{D}\right)$ sub-part representatives send a message up $T$ once it is easy to see that the algorithm remains correct but uses $O(n)$ messages total.
 
Moreover, since \Cref{cor:starJoinRand} provided an efficient means of randomly computing star joinings of sub-part clusters and \Cref{lem:stardivSPClust} stated that if we could compute star joinings of sub-part clusters then we could compute which parts have block number less than $3b$, it is possible to randomly compute in $O(bD \log^2 n + c \log^2 n)$ rounds and $O(m \log n)$ messages which parts have block number larger than $3b$. By \Cref{lem:starJoinUse} repeating \citet{GoranShortcuts}'s ammended algorithm $O(\log n)$ times (removing parts with block number less than $3b$ in each repetition) computes the stated shortcut with the stated round and message complexities.
\end{proof}

Combining \Cref{thm:computePartf} or \Cref{thm:MST} with the now unpacked randomized black boxes yields the randomized algorithm of \Cref{thm:partComputation} or \Cref{thm:mst} respectively.

%Combining \Cref{cor:starJoinRand}, \Cref{thm:randSCut}, \Cref{lem:comDiv}, \Cref{lem:stardivSPClust}, \Cref{thm:MST} and \Cref{thm:computePartf} yields the randomized algorithms of \Cref{thm:partComputation} and \Cref{thm:mst}.%Commenting this out because it's not particularly informative

